CREAK: A Dataset for Commonsense Reasoning over Entity Knowledge

Most benchmark datasets targeting commonsense reasoning focus on everyday scenarios: physical knowledge like knowing that you could fill a cup under a waterfall [Talmor et al., 2019], social knowledge like bumping into someone is awkward [Sap et al., 2019], and other generic situations. However, there is a rich space of commonsense inferences anchored to knowledge about specific entities: for example, deciding the truthfulness of a claim "Harry Potter can teach classes on how to fly on a broomstick." Can models learn to combine entity knowledge with commonsense reasoning in this fashion? We introduce CREAK, a testbed for commonsense reasoning about entity knowledge, bridging fact-checking about entities (Harry Potter is a wizard and is skilled at riding a broomstick) with commonsense inferences (if you're good at a skill you can teach others how to do it). Our dataset consists of 13k human-authored English claims about entities that are either true or false, in addition to a small contrast set. Crowdworkers can easily come up with these statements and human performance on the dataset is high (high 90s); we argue that models should be able to blend entity knowledge and commonsense reasoning to do well here. In our experiments, we focus on the closed-book setting and observe that a baseline model finetuned on existing fact verification benchmark struggles on CREAK. Training a model on CREAK improves accuracy by a substantial margin, but still falls short of human performance. Our benchmark provides a unique probe into natural language understanding models, testing both its ability to retrieve facts (e.g., who teaches at the University of Chicago?) and unstated commonsense knowledge (e.g., butlers do not yell at guests).

==> datasheet.tex <==
\section*{Datasheet for \oursno}
% \appendix
\section{Motivation for Datasheet Creation}
\paragraph{Why was the dataset created?}
Despite their impressive abilities, large-scale pretrained models often fail at performing simple commonsense reasoning. While most benchmark datasets target commonsense reasoning within the context of everyday scenarios, there is a rich, predominantly unexplored space of commonsense inferences that are anchored in knowledge about specific entities. We, therefore, create this dataset to guage how well current pretrained language models are able to perform this type of reasoning and to promote the development of systems that can handle these challenges.

\paragraph{Has the dataset been used already?}
We require all papers reporting on our dataset to submit their results to our dataset website, which will be released upon publication.

\paragraph{Who funded the dataset?}
\michael{TODO}

\section{Dataset Composition}
\paragraph{What are the instances?}
Each instance is a claim about an entity which may be either true or false. These claims are constructed such that validating it requires either knowledge of the entity, common sense reasoning, or both.

\renewcommand{\arraystretch}{1}
\begin{table*}[t]
	\centering
	\small
		\caption{Data statistics of \oursno.}
	\setlength{\tabcolsep}{4pt}
    \centering
	\begin{tabular}{l c c c c c c c c c c}
		%\toprule
		\toprule
		\multicolumn{1}{c}{\multirow{3}{*}{Split}} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\# Claims}& \multicolumn{1}{c}{}  & \multicolumn{1}{c}{Average Length}& \multicolumn{1}{c}{} & \multicolumn{1}{c}{\multirow{3}{*}{\# Unique Entities}} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\multirow{3}{*}{Vocab Size}}\\
		%\cmidrule(r){3-5} \cmidrule(r){7-8} 
		\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Total} & \multicolumn{1}{c}{True} & \multicolumn{1}{c}{False} & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{(\# tokens)}  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}\\
		\midrule
		Train && 10,176 & 5,088 & 5,088 && 10.8  && 2,096 && 19,006 \\
		Dev && \:\:\:1,371 & \:\:\:691 & \:\:\:680 &&  \:\:9.7  && \:\:\:531 && \:\:\:4,520\\
		Test && \:\:\:1,371 & \:\:\:707 & \:\:\:664 && \:\:9.9  && \:\:\:538 && \:\:\:4,620\\
		Contrast && \:\:\:\:\:\:200 & \:\:\:100 & \:\:\:100 && 11.0  && \:\:\:100 && \:\:\:\:\:\:800\\
		\bottomrule 
	\end{tabular}
    \label{tab:datasheet_dataset_counts}
	%\hspace{4pt}
	%\vspace{-10pt}
\end{table*}

\paragraph{How many instances are there?}
Our dataset consists of 13K claims, some of which form a small-scale contrastive evaluation set. A detailed breakdown of the number of instances can be seen in Table~\ref{tab:datasheet_dataset_counts}

\paragraph{What data does each instance consist of?}
Each instance is a human-written claim about a given Wikipedia entity with an associated \texttt{TRUE}/\texttt{FALSE} label of its factually.

\paragraph{Does the data rely on external resources?}
No, all resources are included in our release.

\paragraph{Are there recommended data splits or evaluation measures?}
We include the recommended train, development, and test sets for our datasets. Each split is constructed such that there are no overlapping annotators nor entities between each set. We also include a small contrast set containing minimally edited pairs of examples with opposing labels of factually. The distribution of examples across splits can be seen in Table~\ref{tab:datasheet_dataset_counts}.

\section{Data Collection Process}
\paragraph{How was the data collected?}
We split up data collection into three stages: (1) Identification where annotators are asked to identify whether to the answer to a question depends on its temporal or geographical context. (2) \{Context / Answer\} collection where annotators are asked to identify the answers from additional contexts by providing a brief timeline of answers to temporally dependent questions or valid location/answer pairs for geographically dependent questions. (3) Validation where annotators are presented with all answer timelines or location/answer pairs that were collected in the prior step and are asked to validate or revise each.

\paragraph{Who was involved in the collection process and what were their roles?}
We recruit crowdworkers from Amazon Mechanical Turk to perform the all the annotation steps outlined above.

\paragraph{Over what time frame was the data collected?}
The dataset was collected over a period of April to August 2021.

\paragraph{Does the dataset contain all possible instances?}
We source our list of Wikipedia entities from \citet{Mor_Geva_2021}, who filter for popular entities by measuring the number of contrubutors and backlinkes to each entity. We furthermore allow annotators to select one of five entities to construct an example for. Our sampling process, therefore, filters out a large number of obscure entities which are unfamiliar for crowdworkers. Furthermore, we filter out many simple, purely factoid based claims by disallowing claims 

While we do not cover the entire space of possible entity-centric claims, we promote diversity in our dataset by limiting the total number of claims a single worker can generate to 7\% of any single split. In total, our dataset is comprised of claims that were generated from 684 total crowdworkers.

\paragraph{If the dataset is a sample, then what is the population?}
\oursno represents a subset of all possible entity-centric claims which may require entity-specific knowledge, commonsense, or both to verify. 

\section{Data Preprocessing}

\paragraph{What preprocessing / cleaning was done?}
We do minimal preprocessing on the collected claims, \michael{todo}

\paragraph{Was the raw data saved in addition to the cleaned data?}
We maintain a record of all the original authored claims, as well as an explanation written by each claim's author. 

\paragraph{Does this dataset collection/preprocessing procedure achieve the initial motivation?}
Our collection process indeed achieves our initial goals of creating a dataset that is both diverse and contains entity-centric claims . Using this data, we are able to evaluate how models that are trained on past data generalize to answering questions in the future, asked at the time of our data collection. We recognize, however, that as time goes on, facts will continue to change and will necessitate updating benchmarks with new answers.

\section{Dataset Distribution}
\paragraph{How is the dataset distributed?}
We is availible at \url{https://www.cs.utexas.edu/~yasumasa/entity_commonsense/}.

\paragraph{When was it released?}
Our data and code is currently available.

\paragraph{What license (if any) is it distributed under?}
Our data and code will be available upon publication.

\paragraph{Who is supporting and maintaining the dataset?}
This dataset will be maintained by the authors of this paper. Updates will be posted on the dataset website.

\section{Legal and Ethical Considerations}
\paragraph{Were workers told what the dataset would be used for and did they consent?}
Crowd workers informed of the goals we sought to achieve through data collection. They also consented to have their responses used in this way through the Amazon Mechanical Turk Participation Agreement.

\paragraph{If it relates to people, could this dataset expose people to harm or legal action?}
Our dataset does not contain any personal information of crowd workers; however, our dataset can include incorrect information, or claims about people who already have dedicated Wikipedia pages. We perform extensive quality control and error analysis to minimize the risk due to incorrect labels.

\paragraph{If it relates to people, does it unfairly advantage or disadvantage a particular social group?}
One of our goals in collecting this dataset was to facilitate the development of QA systems that can answer questions from people who live in locations that are poorly represented in current datasets. While our dataset does cover many of these poorly represented locations, we note that it only covers a fraction of the long tail of possible locations. Furthermore, there may be bias in what locations are covered, in part due to what information is available and easily accessible on Wikipedia.
